A Large-Scale 3D Face Mesh Video Dataset via Neural Re-parameterized Optimization

We propose NeuFace, a 3D face mesh pseudo annotation method on videos via neural re-parameterized optimization. Despite the huge progress in 3D face reconstruction methods, generating reliable 3D face labels for in-the-wild dynamic videos remains challenging. Using NeuFace optimization, we annotate the per-view/-frame accurate and consistent face meshes on large-scale face videos, called the NeuFace-dataset. We investigate how neural re-parameterization helps to reconstruct image-aligned facial details on 3D meshes via gradient analysis. By exploiting the naturalness and diversity of 3D faces in our dataset, we demonstrate the usefulness of our dataset for 3D face-related tasks: improving the reconstruction accuracy of an existing 3D face reconstruction model and learning 3D facial motion prior. Code and datasets will be available at https://neuface-dataset.github.io.

==> figures/ablation.tex <==
\begin{figure}
    \centering
    % \vspace{6mm}
    \includegraphics[width=1\linewidth]{ICCV23_3DFace/Figures/source/ablation_spatial_final.pdf}
    %\vspace{-1.5mm}
    \caption{\textbf{Effect of the multi-view consistency loss.} By optimizing our full objectives (Eq.~\colorref{1} in the main paper), the generated meshes are fitted to each of its 2D landmarks and are also multi-view consistent. 
    Views are aligned for the visualization.}
    \vspace{-1mm}
    \label{fig:ablation}
\end{figure}

==> figures/dataset_sample.tex <==
\begin{figure*}[th]
  \centering
  % \fbox{\rule{0pt}{0.5in} \rule{0.9\linewidth}{0pt}}
  \includegraphics[width=\linewidth]{figures/source/wacv_teaser.pdf}
   \caption{\textbf{NeuFace-dataset samples.}
   % 
   % By re-parameterizing face meshes with neural network and optimizing it, 
   % 
   % we leverage NeuFace to
   We annotate
   % automate NeuFace to 
   % automatically 
   % acquire 
   accurate and spatio-temporally consistent 
   % face mesh pseudo-labels 
   % \yw{
   3D face mesh pseudo-labels
   for 
   % 
   large-scale 2D video datasets. 
   % 
   Video frames and paired face meshes
   % annotations
   are visualized as follows; 
   MEAD~\cite{kaisiyuan2020mead} (col.1-2) , VoxCeleb2~\cite{voxceleb2} (col.3-4) and CelebV-HQ~\cite{zhu2022celebvhq} (col.5-8).
   % 
   % Such large-scale 2D datasets contain diverse visual attributes,
   % \eg, wide variety of races, hair styles, backgrounds and natural facial expressions. 
   % 
   % We leverage the acquired datasets for training off-the-shelf 
   % face mesh regressor, DECA~\cite{DECA:Siggraph2021}, via auxiliary
   % % additionally designed 
   % 3D supervision.
   (More samples in \emph{video} can be found in the supplementary material.)
   % and generated self-supervision, 
   % NeuFace 
   }
   \label{fig:dataset_sample}
\end{figure*}

==> figures/deca_issue.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.75\linewidth]{KRAFTON_CVPR2023/Figures/source/intro_poses.pdf}
    \vspace{-6mm}
    \caption{\textbf{(Figures need to be fixed) The results of 3D mesh reconstruction with DECA of the same face image taken with different camera views.}}
    \label{fig:deca_issue}
\end{figure}

==> figures/now_benchmark.tex <==
% \newcommand{\blank}[1]{\hspace*{#1}}
% \begin{figure*}[tp]
\begin{figure}
    \centering
    \small
    \begin{tabular}{c c}
        \blank{-0.5cm}
        \includegraphics[width=0.45\linewidth]{KRAFTON_CVPR2023/Figures/source/now_coarse_placeholder.pdf}
        &
    % \begin{tabular}{c c c}
        % \small{(a)} && \small{(b)}\\
        % \vspace{2mm}
        % \resizebox{0.59\linewidth}{!}{%
        \blank{-0.5cm}
        \raisebox{1.5\height}{
        \resizebox{0.5\linewidth}{!}{%
        \begin{tabular}{l ccc} 
        \toprule
        & \multicolumn{3}{c}{Error[mm] ($\downarrow$)}\\
        \cmidrule{2-4}
        Method & Median & Mean & Std \\
        \cmidrule{1-4}
        DECA\textsubscript{STREAM-2D} & 1.30 & 1.63 & 1.38 \\
        DECA\textsubscript{STREAM-3D} & \textbf{1.27} & \textbf{1.60} & \textbf{1.36} \\
        \bottomrule
        \end{tabular}
        }}
    \end{tabular}
        % }
    % \end{tabular}
    % \blank{-0.2cm}
    % (a) Comparisons of rendered meshes over different views 
    % \blank{2.0cm}
    % (b) Comparisons of cross-view vertex distance
    \caption{\textbf{Results for the NoW benchmark.} We compare the 3D face reconstruction performance of the model trained with and without our 3D auxiliary supervision, computed using STREAM-dataset. Using 3D annotations on our dataset and corresponding losses improve the accuracy of 3D face mesh reconstruction.}
    \label{fig:now}
    % \vspace{-3mm}
\end{figure}

==> figures/now_qual.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/source/now_qual.pdf}\vspace{-3mm}
    \caption{\textbf{Qualitative improvement on 3D face reconstruction.}
    % 
    We enhance the
    existing
    % monocular
    face 
    reconstruction model 
    % mesh regressor
    with our dataset.
    %
    NeuFace-dataset helps the model 
    % achieve
    reconstruct
    more occlusion robust and expressive
    % regress better image-fitted 
    % more accurate
    % and well-fitting
    3D faces than the original model.
    % 
    Green and red dots denote visible and invisible 3D landmarks, respectively.}
    \label{fig:nowqual}
\end{figure}

==> figures/teaser_sample.tex <==
%%%ORIGINAL VERSION
% \begin{figure}[ht]
%   \centering
%     \includegraphics[width=0.9\linewidth]{ICCV23_3DFace/Figures/source/teaser_4.pdf}
%     % \vspace{-2mm}
%     % \captionof{figure}{
%     \caption{\yw{\textbf{NeuFace} is a 3DMM annotation method for videos via neural re-parameterization of 3DMMs. We annotate spatio-temporally consistent 3DMM pseudo-labels for large-scale 2D face video datasets (NeuFace-dataset) and investigate its usefulness, diversity and naturalness with various applications.}}
%    \label{fig:dataset_sample_teaser}
% \end{figure}



%%%REVISED VERSION
\definecolor{Gray}{gray}{0.88}
\begin{figure}[ht]
  \centering
    \includegraphics[width=0.8\linewidth]{figures/source/teaser.pdf} \\
    \vspace{1.5mm}
    \resizebox{1\linewidth}{!}{
    \begin{tabular}{l c@{\,\,\,}c@{\,\,\,\,}c@{\,\,\,\,}c@{\,\,}c}
\toprule
% \multirow{2}{*}{Dataset}&\multirow{2}{*}{\# seq. [K]}&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# id. \\ \end{tabular}}&\multirow{2}{*}{\# views [max]}&\multirow{2}{*}{Duration [hrs]}&\multirow{2}{*}{Env.}\\
Dataset&\# seq. [K]&\# id&\# max views &Dur. [hrs]&Env.\\
% \multirow{2}{*}{Dataset}&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# seq.  \\ $[$ K $]$ \end{tabular}}&\multirow{2}{*}{\# id.}&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# views\\ $[$ max $]$\end{tabular}}&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Duration\\ $[$ hrs $]$\end{tabular}}&\multirow{2}{*}{Env.}\\
% &&&\\
\cmidrule{1-6}
% MEAD$_{\text{3D}}$ & 210K & 48 & 7 & 25hrs & Lab\\
% VoxCeleb2$_{\text{3D}}$ & 1M & 6,000 & 1 & 2,000hrs & Wild\\
% CelebV-HQ$_{\text{3D}}$ & 35K & 15,000 & 1 & 65hrs & Wild\\

% \cmidrule{1-6}
% \bottomrule
\multicolumn{4}{l}{\textbf{Existing 3D face video datasets}}\\
BIWI 3D~\cite{fanelli20103} & 1.1 & 14 & 1 & 1.4 & Lab. \\
COMA~\cite{COMA:ECCV18} & 0.15 & 12 & 4 & 0.1 & Lab. \\
VOCASET~\cite{VOCA2019} & 0.5 & 12 & 4 & 0.5 & Lab.\\
% MICA (only video)~\cite{MICA:ECCV2022} & 1.5 & 200 & 1 & 1.5 & Lab.\\
\cmidrule{1-6}
% \multicolumn{4}{l}{\textbf{Our dataset}}\\
\rowcolor{Gray}
\textbf{NeuFace-dataset (Ours)} & \textbf{1,245} & \textbf{21,048} & \textbf{7} & \textbf{2,090} & \textbf{Wild + Lab.}\\
\quad $\vdash$ NeuFace$_{\text{MEAD}}$ & 210 & 48 & 7 & 25 & Lab.\\
\quad $\vdash$ NeuFace$_{\text{VoxCeleb2}}$ & 1,000 & 6,000 & 1 & 2,000 & Wild\\
\quad $\vdash$ NeuFace$_{\text{CelebV-HQ}}$ & 35 & 15,000 & 1 & 65 & Wild\\
\bottomrule
% \vspace{2mm}
\end{tabular}
    }
    \caption{[Top] Overview of \textbf{NeuFace}, which is a 3D face pseudo-annotation method for videos via neural re-parameterization.
    % (Top).
    % of 3DMMs. 
    % 
    We annotate spatio-temporally consistent 3D 
    face meshes 
    % pseudo-labels 
    for 
    curating existing large-scale 2D face videos, called NeuFace-dataset,
    and investigate its usefulness
    % , diversity, and naturalness 
    with various applications.
    % 
    [Bottom] Comparison between existing datasets and our \textbf{NeuFace-dataset}.
    Our dataset consists of 
    NeuFace$_{\text{MEAD}}$, NeuFace$_{\text{VoxCeleb2}}$, and NeuFace$_{\text{CelebV-HQ}}$,
    and is significantly richer
    % regarding
    % in terms of 
    than
    % both scale and diversity compared to 
    the existing 
    % 3DMM 
    datasets in terms of the scale, diversity and naturalness. 
    $\emph{Abbr.}$ \{seq.: sequences, id.: identities, Dur.: duration, Env.: environment\}
    }
    % \vspace{-3mm}
   \label{fig:dataset_sample_teaser}
\end{figure}

==> main/0_abstract.tex <==
\begin{abstract}
We propose NeuFace, a 3D face mesh pseudo
annotation method on videos via neural re-parameterized
optimization.
% with spatio-temporal consistency.
% 
% We design \oh{an} \ohc{novel} optimization method that fits the neural re-parameterized 3D face meshes on videos.
% % 
% By leveraging spatio-temporal cues inherent in face videos, 
% we develop simple-yet-effective multi-view and temporal consistency losses.
% \yw{
% Though substantial progress on 3D face 
% reconstruction models 
% has been made, 
Despite the huge progress in 3D face reconstruction methods, 
generating reliable 3D face labels for in-the-wild dynamic videos 
remains challenging.
% }
% , and
Using NeuFace optimization, we annotate the per-view/-frame accurate and consistent face meshes on large-scale face videos, called the NeuFace-dataset.
% 
% 
% \yw{
We investigate how
 % of 
% STREAM optimization 
neural re-parameterization
helps to reconstruct
% ing
image-aligned 
% expressive
facial details on 3D meshes
via gradient analysis.
% }
% and 
 % the data dependency 
% In experiments, we 
% validate 
% and demonstrate 
% the efficacy of the proposed optimization.
% and the benefit of STREAM-dataset. 
% 
% We exploit 
% large-scale, 
By exploiting the naturalness and diversity of 3D faces in our dataset,
% of our dataset,
we demonstrate the usefulness
% excellence
of our dataset for
% for 
% in many 
3D face-related tasks: 
% \eg, 
improving the reconstruction accuracy 
% benchmark performance 
of an
% the 
existing 3D face reconstruction model and learning 3D facial motion prior.
% facial mesh regression model.
%
\postechred{Code and datasets will be publicly available if accepted}.
\end{abstract}

==> main/4_data.tex <==
% \input{figures/dataset_sample}

% \input{figures/voca}


\section{The NeuFace-dataset}
%
We introduce the NeuFace-dataset and its acquisition (\Sref{sec: dataset}), and 
% which is 
% the first large-scale 
% % 3D mesh pseudo ground-truth 
% 3D face mesh pseudo-labeled
% dataset 
% constructed by our proposed method, NeuFace.
% ~(\Sref{sec:NeuFace}).
% 
% we 
evaluate the fidelity of our dataset on
% in terms of
its spatio-temporal consistency and 2D landmark accuracy (\Sref{sec: eval}).




\subsection{Acquisition of the NeuFace-dataset}
\label{sec: dataset}
The NeuFace-dataset provides accurate and spatio-temporally consistent 
% mesh annotations 
face meshes of
% the
existing large-scale 2D face video datasets;
% 
MEAD~\citep{kaisiyuan2020mead}, VoxCeleb2~\citep{voxceleb2}, and CelebV-HQ~\citep{zhu2022celebvhq}. 
Our datasets are denoted with 
NeuFace\textsubscript{$\{*\}$}
% $[\cdot]_{\text{3D}}$ 
and summarized in \Tref{tab:data_stat}.
% 
% emotional 
% MEAD is a synchronized multi-view
% % and temporally-synchronized
% % audio-visual 
% dataset containing 
% % high-quality 
% talking head videos with diverse emotion categories and expression levels.
% % 
% VoxCeleb2 is a single-view in-the-wild dataset containing over a million 
% short video clips of over 6,000 speakers.
% % 
% CelebV-HQ is a recently released high-resolution single-view in-the-wild video dataset, 
% featuring diverse facial attributes, actions, emotions, and appearances.
% % 
We optimize our full objective (\Eref{eq:obj}) to acquire FLAME 
% annotations
meshes
for the datasets with a multi-view camera setup, \eg, MEAD.
% , which is in a multi-view camera setup. 
% 
Otherwise, we optimize (\Eref{eq:obj}) with $\lambda_{\text{view}}{=}0$.
% , to obtain pseudo-ground truth 3D face sequences.
% 
% After acquisition, we 
% conduct human verification to filter out noisy face meshes, and achieve ${<}0.1\%$ failure rate.
% \yw{
% During acquisition, w
% 
% For the human verification, 
% we check
We automatically discard the sequences if the optimization yields 
out-of-distribution shape parameters, \ie, the L2-norm of 
shape parameters deviates largely from
the 
% mean of 
pre-built distribution~\citep{FLAME:SiggraphAsia2017}, $\lVert\boldsymbol{\beta}\rVert_2{>}1.0$, or 
% 
% noisy 
% We further discard the sequences 
if the 2D landmark detector~\citep{FAN} fails to capture the faces.
% in the video. 
After subsequent human verification, 
% and 
% NeuFace optimization 
the NeuFace-dataset
achieves ${<}0.1\%$ of failure rate
% } 
on upon criteria, supporting the reliable quality of our dataset.
% or (2) the norm of optimized shape parameters exceed certain extent~\citep{FLAME:SiggraphAsia2017}.
% \input{tables/mica}
% Our datasets are denoted with 
% NeuFace\textsubscript{$*$}
% % $[\cdot]_{\text{3D}}$ 
% and summarized in \Fref{fig:dataset_sample_teaser}.
% 

The NeuFace-dataset is, namely, the largest 3D face mesh pseudo-labeled dataset
% 3D face mesh annotated dataset,
% annotated dataset, 
in terms of the scale, naturalness, and diversity of facial attributes, emotions, and backgrounds. 
% 
The NeuFace-dataset provides high-quality 3D face meshes
% pseudo-annotations
for not only multi-view captured videos but also large-scale ``in-the-wild'' video datasets (see \Fref{fig:teaser_data}).
% for visualized samples).






% \input{tables/2_quantitative}

% \input{tables/mica}

\subsection{Evaluation of the NeuFace-dataset} \label{sec: eval}
% \vspace{-3mm}

% For the general usage of the NeuFace-dataset, we need to verify its fidelity.
% Here, w
We assess the fidelity of our dataset in terms of 
% of our dataset.
% in terms of
spatio-temporal consistency and landmark accuracy. 
% 
% \yw{
% asdf
% To compare the quality of the generated mesh annotations, 
We make competing datasets using various methods and compare the quality of the generated mesh annotations.
% 
First, we compose the strong baseline, Base-dataset, by fitting FLAME with \Eref{eq:baseline}. 
% Base-dataset is built on the standard protocol of the original FLAME fitting codebase with the 3DMM prior and  
%
We also utilize pre-trained DECA and EMOCA as mesh annotators and built DECA-dataset and EMOCA-dataset, respecitvely.
% 
Finally, we build two versions of our dataset, \ie, NeuFace-D, and NeuFace-E, where each dataset is generated via \Eref{eq:obj} with DECA and EMOCA for the neural re-parameterization $\Phi_{\mathbf{w}}$, respectively.
% }
%
%As 
% Note that /
% As aforementioned, 
% As off-the-shelf neural models can 
% serve as strong pseudo-label generators,
% % Thus, 
% we build the solid baseline dataset acquired by the 
% recent 3D face reconstruction model DECA~\citep{DECA:Siggraph2021}, 
\begin{comment}
To build a large-scale
% strong
baseline dataset, we use 
% an existing 
% off-the-shelf 
% neural model
pre-trained
DECA~\citep{DECA:Siggraph2021} as a pseudo-annotator and create the Base-dataset 
using the same video datasets as ours.
As the whole dataset is large-scale, we sample 10,000 annotated mesh sequences 
from both the NeuFace-dataset and the Base-dataset as the validation sets.
% , 
% called Base-dataset.e
% , MEAD, VoxCeleb2 and Celebv-HQ,
% and denote it as Na\"ive-dataset. 
% 
% By comparing 
% our dataset with Na\"ive dataset,
% The goal here
Our goal here
% aim
is to highlight the 
favorable 
quality 
% and practicality
% and spatio-temporal consistency 
of our dataset over the Base-dataset.
% , 
% 
% showing practicability for the general usage of our dataset.
\end{comment}

% how our dataset 

% in terms of
% spatio-temporal consistency and landmark accuracy, 
% The goal here is to demonstrate why
% our dataset 
% how 
% our optimization generate
% We compare our dataset and 
% Na\"ive-dataset for sampled 
% 10,000 validation sequences.
% For the general usage of the NeuFace-dataset, we need to verify its fidelity.
% We evaluate the NeuFace-dataset in terms of
% spatio-temporal consistency and landmark accuracy. 
% %
% We build the baseline dataset acquired by the 
% recent neural 3D face reconstruction model, e.g., DECA~\citep{DECA:Siggraph2021}, 
% with the same 2D video datasets, MEAD, VoxCeleb2 and Celebv-HQ,
% and denote it as Na\"ive-dataset. 
% We compare our dataset and 
% Na\"ive-dataset for sampled 
% 10,000 validation sequences.
% of 
% 
% sequences as 
% sets of each dataset.

% We compare with the dataset acquired by na\"ively regressing the meshes 
% % 
% from the off-the-shelf neural 3D face reconstruction model,
% % 3D face mesh regression network, 
% \eg, DECA~\citep{DECA:Siggraph2021}, and denote it as Na\"ive-dataset.
% %

% of MEAD~\citep{kaisiyuan2020mead}, VoxCeleb2~\citep{voxceleb2}, and CelebV-HQ~\citep{zhu2022celebvhq},
% respectively, 
% for the comparison.}

% 



\input{figures/spatial_qual}



\paragraph{Multi-view consistency}
We visualize the predicted
% rendered
meshes over different views
% , as 
in 
%\Fref{fig:spatial_qual}~(a).
\Fref{fig:spatial_qual}, where 
per-view independent estimations
% meshes
are presented, not a single merged one.
% \kim{
% Note that t
% The meshes from both datasets are non-merged but independently predicted from each viewpoint.
% of the viewpoints.}
We
% can clearly 
verify that the NeuFace-D-dataset contains multi-view consistent meshes compared to the DECA-dataset, especially near the mouth region.
% 
See supplementary material for the comparison of the EMOCA-dataset and NeuFace-E-dataset. 
% In particular, the Base-dataset reconstructs the mouth 
% poses 
% with huge discrepancies across the views, while ours are
% relatively 
% more consistent.
%
% To quantitatively measure
% the multi-view consistency of meshes in 
% our dataset, 
As a quantitative
% multi-view consistency 
measure,
we 
% quantitatively, we 
% propose 
compute the cross-view vertex distance (CVD), \ie, the vertex distance between two different views, $i$ and $j$, in the same frame $f$: ${\lVert \mathbf{M}_{f,i}{-}\mathbf{M}_{f,j} \rVert}_{1}$. 
We compare the averaged CVD of all views in \Tref{evaluation_results}.
% Note that 
CVD is only evaluated on the 
%validation samples of the 
MEAD dataset, which is in a multi-camera setup.
While the DECA-/EMOCA-dataset results in high CVD, the NeuFace-dataset shows significantly lower CVD on overall views.
% 



\paragraph{Temporal consistency}
We extend the Motion Stability Index
(MSI)~\citep{ling2022stableface} to $\text{MSI}_\text{3D}$
and evaluate the temporal consistency of each dataset.
% 3D face meshes. 
% 
% We compute 
MSI\textsubscript{3D} computes a reciprocal of the motion 
acceleration variance of either 3D landmarks or 
vertices
% obtained from the face meshes 
and 
quantifies facial motion 
stability 
for a given $N_{F}$ frame video, $\{\mathbf{I}_{f}\}^{N_{F}}_{f=1}$,
as 
$\text{MSI}_\text{3D}(\{\mathbf{I}_{f}\}^{N_{F}}_{f=1}){=}\tfrac{1}{K}\sum_{i}\tfrac{1}{\sigma(\mathbf{a}^i)}$,
% 
% \begin{equation*}
% \label{eq:msi_2}
%     \text{MSI\textsubscript{3D}}(\mathbf{I}_{1:N_{F}}) = \frac{1}{K}\sum_{i=1}^{K}\frac{1}{\sigma(\mathbf{a}^i)}\, ,
% \end{equation*}
% 
where $\mathbf{a}^i$ denotes the 3D motion acceleration of $i$-th 3D landmarks or vertices, 
$\sigma(\cdot)$ 
% denotes
% means measuring
% taking
the temporal variance, 
% marginalized 
% over time-axis 
and $K$ the number of 
% 3D points of interest, \eg, 
landmarks or vertices.
% dynamics.
% 
If the mesh sequence has 
% that is, 
small temporal jittering, 
\ie, low motion variance,
it has a high $\text{MSI}_\text{3D}$ value. 
% 
% Therefore, we compute
% % \yw{consider}
% % define 
% the MSI\textsubscript{3D} of given 
% % , as the reciprocal of the variance of motion acceleration 
% as follows: 
% selected 3D landmarks. 
% 
We 
% can 
compute $\text{MSI}_\text{3D}$ for landmarks and vertices, \ie, $\text{MSI}_\text{3D}^{\text{L}}$ and $\text{MSI}_\text{3D}^{\text{V}}$, respectively.
% by replacing
% as changing 
% $\mathbf{J}_{t}^i$ with $\mathbf{M}_{t}^i$, where $\mathbf{M}_{t}^i$ denote $i$-th vertex at time $t$.
% step t.
% 
\Tref{evaluation_results} shows the 
% scores of 
% MSI$_{\text{3D}}$ on 3D landmarks and vertices 
$\text{MSI}_\text{3D}^{\text{L}}$ and $\text{MSI}_\text{3D}^{\text{V}}$
averaged over the validation sets. 
% 
For the VoxCeleb2 and CelebV-HQ splits, the NeuFace-D/E-dataset outperform 
the 
% DECA/EMOCA-dataset
other datasets
% by a factor of three to four 
in 
both MSI\textsubscript{3D}s.
% metrics.
% $\text{MSI}_\text{3D}^{\text{L}}$ and $\text{MSI}_\text{3D}^{\text{V}}$.
% MSI$_{\text{3D}}$ scores for 3D landmarks and vertices.
% 
Remarkably, we have 
% a score 
improvements on MSI\textsubscript{3D} 
% of
more than 20 times in MEAD.
% 
We postulate that the multi-view consistency loss 
% alleviates
also strengthens the temporal consistency for MEAD.
%
In other words, our 
% spatio-temporal
losses would be mutually helpful when jointly optimized.
% for 
% annotating
% generating high-quality 3D face mesh pseudo-labels. 
% 
We discuss it through loss ablation studies in the supplementary material.
% See supplementary for ablation studies on loss terms.

% \input{tables/2_quantitative}

\input{tables/2_quantitative}

\paragraph{2D landmark accuracy}
% One 
A trivial solution to obtain
% achieve
low CVD and high MSI\textsubscript{3D} is to 
regress the same mean face meshes 
across 
% over different 
views and frames regardless of the input image.
To verify such occurrence, we 
% additionally
measure the landmark accuracy between the ground-truth and regressed 2D 
facial
landmarks 
% and the regressed 2D landmarks 
% by 
using the 
% standard 
normalized mean error (NME)~\citep{sagonas2016300}.
% As summarized in \Tref{evaluation_results}, 
The NeuFace-D/E-dataset outperform the 
other datasets in NME (see \Tref{evaluation_results}), \ie, contain spatio-temporally consistent and accurately landmark-aligned meshes.
% on all the validation sets (see \Tref{evaluation_results}).
% These results not only show that our method produces meshes with accurate landmarks but also support the validity of the proposed method, not falling into trivial solutions.
% These results show that 
% Thus, the NeuFace-dataset 
% produces
% contains
% spatio-temporally consistent meshes with accurately landmark-aligned meshes.
% ,
% on the input image
% , 
% not falling into a 
% without 
% trivial solution.

% \input{tables/mica}



% \subsection{Evaluation of the NeuFace-dataset} \label{sec: eval}


\input{tables/mica}

\paragraph{NeuFace vs. MICA${+}$T}
% 
We further verify the favorable quality of NeuFace-datasets by comparing it with 
the meshes obtained by the state-of-the-art method, MICA with a tracker~\citep{MICA:ECCV2022} (MICA${+}$T).
% 
% Since 
% MICA encoder does not infer facial poses from the image; thus, we could not use it as a backbone of our system.
% for NeuFace.
% 
% Instead, we compare with an advanced variant, MICA with a tracker, 
% 
MICA${+}$T jointly optimizes 3DMM, cameras, and textures with landmark and photometric losses, and statistic regularizers.
% via differentiable rendering.  
% 
In \Tref{tab:mica}, NeuFace performs better than MICA${+}$T in CVD \& NME with comparable MSI.
% 
Also, faster optimization makes NeuFace preferable when annotating large-scale videos.
% 






==> tables/1_datasets.tex <==
% \newcolumntype{a}{>{\columncolor{Gray}}c}

\begin{table}[t]
\centering
\resizebox{0.65\linewidth}{!}{%
% \begin{tabular}{l ccccc}
% \begin{tabular}{l c@{\quad}c@{\quad}c@{\quad}c@{\quad}c}
\begin{tabular}{l c@{\,\,\,}c@{\,\,\,\,}c@{\,\,\,\,}c@{\,\,}c}
\toprule
% \multirow{2}{*}{Dataset}&\multirow{2}{*}{\# seq. [K]}&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# id. \\ \end{tabular}}&\multirow{2}{*}{\# views [max]}&\multirow{2}{*}{Duration [hrs]}&\multirow{2}{*}{Env.}\\
Dataset&\# seq. [K]&\# id&\# max views &Dur. [hrs]&Env.\\
% \multirow{2}{*}{Dataset}&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# seq.  \\ $[$ K $]$ \end{tabular}}&\multirow{2}{*}{\# id.}&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}\# views\\ $[$ max $]$\end{tabular}}&\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Duration\\ $[$ hrs $]$\end{tabular}}&\multirow{2}{*}{Env.}\\
% &&&\\
\cmidrule{1-6}
% MEAD$_{\text{3D}}$ & 210K & 48 & 7 & 25hrs & Lab\\
% VoxCeleb2$_{\text{3D}}$ & 1M & 6,000 & 1 & 2,000hrs & Wild\\
% CelebV-HQ$_{\text{3D}}$ & 35K & 15,000 & 1 & 65hrs & Wild\\

% \cmidrule{1-6}
% \bottomrule
\multicolumn{4}{l}{\textbf{Existing facial motion capture dataset}}\\
BIWI 3D~\cite{fanelli20103} & 1.1 & 14 & 1 & 1.4 & Lab. \\
COMA~\cite{COMA:ECCV18} & 0.15 & 12 & 4 & 0.1 & Lab. \\
VOCA~\cite{VOCA2019} & 0.5 & 12 & 4 & 0.5 & Lab.\\
% MICA (only video)~\cite{MICA:ECCV2022} & 1.5 & 200 & 1 & 1.5 & Lab.\\
\cmidrule{1-6}
% \multicolumn{4}{l}{\textbf{Our dataset}}\\
\rowcolor{Gray}
\textbf{STREAM-dataset (Ours)} & \textbf{1,245} & \textbf{21,048} & \textbf{7} & \textbf{2,090} & \textbf{Wild + Lab.}\\
\quad $\vdash$ MEAD$_{\text{3D}}$ & 210 & 48 & 7 & 25 & Lab.\\
\quad $\vdash$ VoxCeleb2$_{\text{3D}}$ & 1,000 & 6,000 & 1 & 2,000 & Wild\\
\quad $\vdash$ CelebV-HQ$_{\text{3D}}$ & 35 & 15,000 & 1 & 65 & Wild\\
\bottomrule
% \vspace{2mm}
\end{tabular}
}
\caption{
\textbf{3D face video datasets comparison.} Our STREAM-dataset consists of MEAD$_{\text{3D}}$, VoxCeleb2$_{\text{3D}}$, and CelebV-HQ$_{\text{3D}}$. It significantly outperforms the other 3D face video datasets in both quantity and quality. The symbol \# denotes the number. $\emph{Abbr.}$ seq.: sequences, id.: identities, Dur.: duration, Env.: environment.
}\vspace{-3mm}
\label{tab:dataset}
\end{table}


==> tables/3_Retrain_quan.tex <==
\begin{table}[t!]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l c@{\quad}c@{\quad}c cccc}
  \toprule
    & \multicolumn{3}{c}{NoW benchmark~\cite{RingNet:CVPR:2019}} & \multicolumn{4}{c}{MEAD~\cite{kaisiyuan2020mead}} \\
    \cmidrule(lr){2-4} \cmidrule(lr){5-8} 
    \multicolumn{1}{c}{Method} & Median & Mean & Std & \multicolumn{1}{c}{CVD$\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk}$\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx}$\uparrow$} & \multicolumn{1}{c}{NME$\downarrow$} \\
  \cmidrule{1-8}
\multicolumn{1}{l}{DECA\textsubscript{STREAM,2D}} & 1.30 & 1.63 & 1.38 & 0.152 & 0.007 & 0.011 & 3.95 \\
\multicolumn{1}{l}{DECA\textsubscript{STREAM,3D}} & \textbf{1.27} & \textbf{1.60} & \textbf{1.36}  & \textbf{0.132} & \textbf{0.018} & \textbf{0.026} & \textbf{3.64} \\
    \bottomrule
  \end{tabular}}
  % \vspace{3mm}
  \caption{\textbf{Quantitative evaluation of DECA trained w/ STREAM-dataset.}
  % We 
  We evaluate the accuracy and spatio-temporal consistency of DECA\textsubscript{STREAM,2D/3D} for various datasets.
  DECA\textsubscript{STREAM,3D} shows improved 3D mesh and 2D landmark reconstruction accuracy than DECA\textsubscript{STREAM,2D}.
  % , on 
  % we measure the 3D reconstruction error computed on 
  % NoW benchmark dataset~\cite{RingNet:CVPR:2019} and MEAD~\cite{kaisiyuan2020mead}, respectively.
  % 
  We further analyze the CVD and MSI\textsubscript{3D} of the reconstructed meshes on the MEAD.
  % 
  DECA trained with our 3D annotations show remarkable enhancement on all aspects, noticeably about $2.5\times$ gain on temporal consistency. 
  }
  % \vspace{-3mm}
  \label{retrain}
  % , multi-view consistency (CVD) and temporal consistency (MSI\textsubscript{3D}), along with the 2D landmark accuracy (NME~\cite{sagonas2016300}) and show that STREAM significantly outperforms the competing method, DECA in overall metrics. CVD and NME are lower the better, and MSI is higher the better. $\emph{Abbr.}$ lmk: landmark, vtx: vertex.}
% \label{evaluation_results}
\end{table}


==> tables/rebuttal_fd_apd.tex <==
% \begin{table}[t!]
%   \centering
%   \resizebox{0.8\linewidth}{!}{
%   \begin{tabular}{l |cc|cc|cc}
%   \toprule
%   % &\multicolumn{2}{c}{Methods} \\
%   % \cmidrule(lr){2-3} 
%    & \multicolumn{2}{c|}{\orange{\textbf{VOCASET}}} & \multicolumn{2}{c|}{\greencap{\textbf{MEAD}}} & \multicolumn{2}{c}{\blueyw{\textbf{VoxCeleb2}}}\\
%    \cmidrule(lr){2-7} 
%    & Generate & Sample & Generate & Sample & Generate & Sample \\
%   \cmidrule(lr){1-7} 
%   FD $\downarrow$ & 420.92 & \orange{\textbf{290.38}} & 78.99 & \greencap{\textbf{77.16}} & 31.32 & - \\ 
%   \cmidrule(lr){1-7} 
%   APD [\emph{cm}] $\uparrow$ & - & 6.56 & 3.56 & \greencap{\textbf{22.26}}& \blueyw{\textbf{52.69}} & 38.66 \\
%   % MICA & 0.xxx & 0.xxx & 0.xxx & x.xx\\
%   % NeuFace (ours) & \textbf{0.103}  & \textbf{0.206} &\textbf{0.305} & \textbf{2.58} \\
%   \bottomrule
%   \end{tabular}}
%   \vspace{1mm}
%   \caption{Motion quality: HuMoR generated vs. dataset sampled}
%   \vspace{-5mm}
%   % }
%   \label{tab:fd_apd}
% \end{table}


 

\begin{table}[t!]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l |cc|cc|cc}
  \toprule
  % &\multicolumn{2}{c}{Methods} \\
  % \cmidrule(lr){2-3} 
   & \multicolumn{2}{c|}{\orange{\textbf{VOCASET}}} & \multicolumn{2}{c|}{\greencap{\textbf{MEAD}}} & \multicolumn{2}{c}{\blueyw{\textbf{VoxCeleb2}}}\\
   \cmidrule(lr){2-7} 
   & FD $\downarrow$ & APD [\emph{cm}] $\uparrow$ & FD $\downarrow$ & APD [\emph{cm}] $\uparrow$ & FD $\downarrow$ & APD [\emph{cm}] $\uparrow$ \\
  \cmidrule(lr){1-7} 
  Generated & 420.92 & - & 78.99 & 3.56 & 31.32 & \blueyw{\textbf{52.69}} \\ 
  \cmidrule(lr){1-7} 
  Upper-bound (Sampled) &  \orange{\textbf{290.38}} & 6.56 & \greencap{\textbf{77.16}} & \greencap{\textbf{22.26}}& - & 38.66 \\
  % MICA & 0.xxx & 0.xxx & 0.xxx & x.xx\\
  % NeuFace (ours) & \textbf{0.103}  & \textbf{0.206} &\textbf{0.305} & \textbf{2.58} \\
  \bottomrule
  \end{tabular}}
  \vspace{1mm}
  \caption{Motion quality: HuMoR generated vs. dataset sampled}
  \vspace{-5mm}
  % }
  \label{tab:fd_apd}
\end{table}


 


==> tables/supp_baseline.tex <==
% \begin{table}[t!]
%   \centering
%   \resizebox{0.98\linewidth}{!}{
%   \begin{tabular}{l cccc}
%   \toprule
% &\multicolumn{4}{c}{MEAD~\cite{kaisiyuan2020mead}} \\
%     \cmidrule(lr){2-5} 
%     \multicolumn{1}{c}{Dataset} & \multicolumn{1}{c}{CVD $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} \\
%   \cmidrule{1-5}
% \multicolumn{1}{l}{Base-dataset}  & {0.209} & 0.011 & 0.016 & 4.65 \\
% \multicolumn{1}{l}{Direct Flame opt. (Eq.~(\colorref{a}))}  & {0.192} & 0.034 & 0.053 & 4.34 \\
% \multicolumn{1}{l}{NeuFace-dataset (ours)} & \textbf{0.103} & \textbf{0.206} & \textbf{0.305} & \textbf{2.58} \\
%     \bottomrule
%   \end{tabular}}
%   % \vspace{1mm}
%   % \caption{\textbf{Quantitative evaluation results.}
%   % We evaluate the quantitative quality of the face meshes reconstructed with STREAM. For sampled sequences for MEAD, VoxCeleb2 and CelebV-HQ, STREAM reliably outperforms the competing method, DECA, for all the aspects; multi-view consistency (CVD), temporal consistency (MSI\textsubscript{3D}) and 2D landmark accuracy (NME~\cite{sagonas2016300}). $\emph{Abbr.}$ $lmk$: landmark, $vtx$: vertex.}
%   \caption{\textbf{Quantitative comparison: Direct FLAME opt. vs. NeuFace.}
%   % \kim{
%   We evaluate the meshes obtained by the direct FLAME opt. (\Eref{eq:baseline})) and meshes in NeuFace-dataset in terms of multi-view consistency (CVD), temporal consistency (MSI\textsubscript{3D}) and the 2D landmark accuracy (NME~\cite{sagonas2016300}). 
%   % 
%   The results show that NeuFace-dataset significantly outperforms the meshes obtained by other solid baselines.
%   % 
%   % 
%   % competing method, DECA, in overall metrics. 
%   % CVD and NME are measured in FLAME canonical coordinate and pixel space, respectively, while MSIs are normalized with min-max scaling.
%   $\emph{Abbr.}$ lmk: landmark, vtx: vertex.}
%   % \vspace{-3mm}
%   % }
%   \label{tab:baseline}
% \end{table}

\begin{table*}[hbt!]
  \label{tab:quant}
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l cccc ccc ccc}
  \toprule
&\multicolumn{4}{c}{MEAD~\cite{kaisiyuan2020mead}} & \multicolumn{3}{c}{VoxCeleb2\cite{voxceleb2}} & \multicolumn{3}{c}{CelebV-HQ~\cite{zhu2022celebvhq}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
    \multicolumn{1}{c}{Dataset} & \multicolumn{1}{c}{CVD $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} \\
  \cmidrule{1-11}
\multicolumn{1}{l}{Base-dataset}  & 0.209 & 0.011&0.016 & 4.65 & 0.028 & 0.044 & 4.78 & 0.012 & 0.018 &5.34\\
\multicolumn{1}{l}{Direct Flame opt. (Eq.~(\colorref{a}))}  & 0.192 & 0.034& 0.053 & 4.34 & 0.034 & 0.056 & 3.32 & 0.030 & 0.047 & 3.65\\
\multicolumn{1}{l}{\textbf{NeuFace-dataset (ours)}} & \textbf{0.103} & \textbf{0.206} & \textbf{0.305} & \textbf{2.58} & \textbf{0.095} & \textbf{0.137} & \textbf{2.19} & \textbf{0.054}&\textbf{0.074}&\textbf{2.55}\\
    \bottomrule
  \end{tabular}}
  % \vspace{1mm}
  % \caption{\textbf{Quantitative evaluation results.}
  % We evaluate the quantitative quality of the face meshes reconstructed with NeuFace. For sampled sequences for MEAD, VoxCeleb2 and CelebV-HQ, NeuFace reliably outperforms the competing method, DECA, for all the aspects; multi-view consistency (CVD), temporal consistency (MSI\textsubscript{3D}) and 2D landmark accuracy (NME~\cite{sagonas2016300}). $\emph{Abbr.}$ $lmk$: landmark, $vtx$: vertex.}
  \caption{\textbf{Quantitative comparison: Direct FLAME opt. vs. NeuFace.}
  % \kim{
  We evaluate the meshes obtained by the direct FLAME opt. (\Eref{eq:baseline}) and meshes in NeuFace-dataset in terms of multi-view consistency (CVD), temporal consistency (MSI\textsubscript{3D}) and the 2D landmark accuracy (NME~\cite{sagonas2016300}). 
  % 
  The results show that NeuFace-dataset significantly outperforms the meshes obtained by other solid baselines.}\vspace{-3mm}
  % }
\label{tab:baseline}
\end{table*}

==> tables/supp_emoca_quant.tex <==
\begin{table*}[th!]
  \centering
  \resizebox{\linewidth}{!}{
  \begin{tabular}{l cccc ccc ccc}
  \toprule
&\multicolumn{4}{c}{MEAD~\cite{kaisiyuan2020mead}} & \multicolumn{3}{c}{VoxCeleb2\cite{voxceleb2}} & \multicolumn{3}{c}{CelebV-HQ~\cite{zhu2022celebvhq}} \\
    \cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
    \multicolumn{1}{c}{Method} & \multicolumn{1}{c}{CVD $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} \\
  \cmidrule{1-11}
\multicolumn{1}{l}{EMOCA~\cite{EMOCA:CVPR:2022}}  & 0.199 & 0.010 &0.016 & 5.42 & 0.003 & 0.004 & 4.77 & 0.005 & 0.007 &5.57\\
\multicolumn{1}{l}{NeuFace-E (ours)} & \textbf{0.104} & \textbf{0.209} & \textbf{0.312} & \textbf{2.28} & \textbf{0.028} & \textbf{0.048} & \textbf{2.38} & \textbf{0.053}&\textbf{0.077}&\textbf{2.86}\\
    \bottomrule
  \end{tabular}}
  % \vspace{1mm}
  % \caption{\textbf{Quantitative evaluation results.}
  % We evaluate the quantitative quality of the face meshes reconstructed with STREAM. For sampled sequences for MEAD, VoxCeleb2 and CelebV-HQ, STREAM reliably outperforms the competing method, DECA, for all the aspects; multi-view consistency (CVD), temporal consistency (MSI\textsubscript{3D}) and 2D landmark accuracy (NME~\cite{sagonas2016300}). $\emph{Abbr.}$ $lmk$: landmark, $vtx$: vertex.}
  \caption{\textbf{Quantitative comparison: EMOCA vs. NeuFace-E.}
  % \kim{
  % We optimize EMOCA with our optimization pipeline and obtain 3D faces for the validation sets. 
  We evaluate face meshes obtained using NeuFace-E and EMOCA with the metrics, CVD, MSI\textsubscript{3D}, and NME~\cite{sagonas2016300}.
  % multi-view consistency (CVD) and temporal consistency (MSI\textsubscript{3D}), along with the 2D landmark accuracy (NME~\cite{sagonas2016300}). 
  The results show that NeuFace-E significantly outperforms the competing method, EMOCA, in overall metrics. 
  % CVD and NME are measured in FLAME canonical coordinate and pixel space, respectively, while MSIs are normalized with min-max scaling.
  $\emph{Abbr.}$ lmk: landmark, vtx: vertex.
  }
  % \vspace{3mm}
  % }
\label{tab:emocaquant}
\end{table*}

==> tables/supp_loss_ablation.tex <==
\begin{table*}[th]
  \centering
  \resizebox{1\linewidth}{!}{
  \begin{tabular}{ccc cccc ccc ccc}
  \toprule
\multicolumn{3}{c}{NeuFace} &\multicolumn{4}{c}{MEAD~\cite{kaisiyuan2020mead}} & \multicolumn{3}{c}{VoxCeleb2\cite{voxceleb2}} & \multicolumn{3}{c}{CelebV-HQ~\cite{zhu2022celebvhq}} \\
     \cmidrule(lr){1-3} \cmidrule(lr){4-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13}
    \multicolumn{1}{l}{$\mathcal{L}_{\text{2D}}$}&\multicolumn{1}{l}{$\mathcal{L}_{\text{multiview}}$}&\multicolumn{1}{l}{$\mathcal{L}_{\text{temporal}}$} & \multicolumn{1}{c}{CVD $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} \\
  \cmidrule{1-13}
\checkmark&&  & 0.333 & 0.015&0.022 & \textbf{2.44} & 0.001 & 0.001 & 2.71 & 0.001 & 0.003 &3.88\\
\checkmark&\checkmark&  & 0.110 & 0.015&0.023 &2.49 & - & - & - & - & - & -\\
% \checkmark&&\checkmark& 0.209 & 0.011&0.016 & 4.65 & - & - & - & - & - & -\\
\checkmark&&\checkmark& 0.294 & 0.176&0.250 & 2.56 & \textbf{0.095} & \textbf{0.137} & \textbf{2.19} & \textbf{0.54} & \textbf{0.074} & \textbf{2.55}\\
% \checkmark&\checkmark&\checkmark& \textbf{0.103} & \textbf{0.206} & \textbf{0.305} & \textbf{2.58} & \textbf{0.095} & \textbf{0.137} & \textbf{2.19} & \textbf{0.054}&\textbf{0.074}&\textbf{2.55}\\
\checkmark&\checkmark&\checkmark&\textbf{0.103} & \textbf{0.206} & \textbf{0.305} & 2.58 & - & -& - & -&-&-\\
% \hline
\cmidrule{1-13}
\multicolumn{3}{c}{DECA~\cite{DECA:Siggraph2021}}  & 0.209 & 0.011&0.016 & 4.65 & 0.028 & 0.044 & 4.78 & 0.012 & 0.018 &5.34\\
    \bottomrule
  \end{tabular}}
  % \vspace{1mm}
  \caption{\textbf{Ablation results on the different loss functions.} We evaluate the effect of our proposed spatio-temporally consistent losses by changing the configurations of the loss combinations. Optimizing full loss functions shows favorable results on CVD and NME while outperforming MSI compared to other configurations. 
  We can not analyze the effect of $\mathcal{L}_{\text{multiview}}$ for VoxCeleb2 and CelebV-HQ since they are taken in the single-camera setup. 
  We provide the results from DECA~\cite{DECA:Siggraph2021} for comparison.
  $\emph{Abbr.}$ lmk: landmark, vtx: vertex.
  }
  % \vspace{3mm}
  % }
\label{tab:ablation}
\end{table*}




% \begin{table*}[hbt!]
%   \centering
%   \resizebox{0.98\linewidth}{!}{
%   \begin{tabular}{l cccc ccc ccc}
%   \toprule
% &\multicolumn{4}{c}{MEAD~\cite{kaisiyuan2020mead}} & \multicolumn{3}{c}{VoxCeleb2\cite{voxceleb2}} & \multicolumn{3}{c}{CelebV-HQ~\cite{zhu2022celebvhq}} \\
%     \cmidrule(lr){2-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
%     \multicolumn{1}{c}{Method} & \multicolumn{1}{c}{CVD $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{NME $\downarrow$} \\
%   \cmidrule{1-11}
% \multicolumn{1}{l}{$\mathcal{L}_{\text{2D}}$}  & 0.209 & 0.011&0.016 & 4.65 & 0.000 & 0.000 & 2.71 & 0.012 & 0.018 &5.34\\
% \multicolumn{1}{l}{$\mathcal{L}_{\text{2D}}{+}\mathcal{L}_{\text{multiview}}$}  & 0.209 & 0.011&0.016 & 4.65 & - & - & - & - & - & -\\
% \multicolumn{1}{l}{$\mathcal{L}_{\text{2D}}{+}\mathcal{L}_{\text{temporal}}$}  & 0.209 & 0.011&0.016 & 4.65 & - & - & - & - & - & -\\
% % \multicolumn{1}{l}{$\mathcal{L}_{\text{2D}}{+}\mathcal{L}_{\text{temporal}}$}  & 0.209 & 0.011&0.016 & 4.65 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1 & 0.1\\
% \multicolumn{1}{l}{STREAM (ours)} & \textbf{0.103} & \textbf{0.206} & \textbf{0.305} & \textbf{2.58} & \textbf{0.095} & \textbf{0.137} & \textbf{2.19} & \textbf{0.054}&\textbf{0.074}&\textbf{2.55}\\
% % \multicolumn{1}{l}{STREAM (ours)} & \textbf{0.103} & \textbf{0.206} & \textbf{0.305} & \textbf{2.58} & - & -& - & -&-&-\\
%     \bottomrule
%   \end{tabular}}
%   % \vspace{1mm}
%   \caption{\textbf{Ablation results on the different loss functions.} We compare the different configurations of our method by changing the combinations of the loss functions. Optimizing all loss functions shows favorable results on CVD and NME while outperforming MSI compared to other configurations.}\vspace{-3mm}
%   % }
% \label{tab:ablation}
% \end{table*}

==> tables/supp_vocaset.tex <==
% \begin{table}[t!]
%   \centering
%   \resizebox{\linewidth}{!}{
%   \begin{tabular}{l cccc}
%   \toprule
% &\multicolumn{4}{c}{VOCASET~\cite{VOCA2019}} \\
%     \cmidrule(lr){2-5} 
%     \multicolumn{1}{c}{Method} & \multicolumn{1}{c}{CVD $\downarrow$} & \multicolumn{1}{c}{MSI\textsubscript{3D, lmk} $\uparrow$} &\multicolumn{1}{c}{MSI\textsubscript{3D, vtx} $\uparrow$} & \multicolumn{1}{c}{MPVE [\emph{mm}] $\downarrow$} \\
%   \cmidrule{1-5}
% \multicolumn{1}{l}{VOCASET (GT)}  & 0.0 & Very good & Very good & $-$ \\
% \cmidrule{1-5}
% \multicolumn{1}{l}{DECA~\cite{DECA:Siggraph2021}}  & bad & bad & bad & bad \\
% \multicolumn{1}{l}{\textbf{NeuFace (ours)}} & \textbf{Good} & \textbf{comparable} & \textbf{comparable} & \textbf{good} \\
%     \bottomrule
%   \end{tabular}}
%   \caption{\textbf{Accuracy of NeuFace optimization on motion capture dataset w/ GT.}
%   % \kim{
%   Given the ground-truth meshes of multi-view motion captured dataset, VOCASET, our NeuFace optimization reconstructs more multi-view consistent (CVD), temporally consistent (MSI's) and vertex-level accurate (MPVE) meshes than the off-the-shelf neural model, DECA. 
%   % 
%   % $\emph{Abbr.}$ lmk: landmark, vtx: vertex.
%   }
%   % \vspace{-3mm}
%   % }
%   \label{tab:vocaset}
% \end{table}




%%%%%%Previous Version, Only MPVE
% \begin{table}[t!]
%   \centering
%   \resizebox{0.6\linewidth}{!}{
%   \begin{tabular}{l cc}
%   \toprule
%   % &\multicolumn{2}{c}{Methods} \\
%   % \cmidrule(lr){2-3} 
%   Method & DECA~\cite{DECA:Siggraph2021} & NeuFace (ours) \\
%   \cmidrule(lr){1-3} 
%   MPVE [\emph{mm}] $\downarrow$ & bad & good \\
%   \bottomrule
%   \end{tabular}}
%   \caption{\textbf{Accuracy of NeuFace optimization on motion capture dataset w/ GT.}
%   % \kim{
%   Given the ground-truth meshes of multi-view motion captured dataset, VOCASET, our NeuFace optimization reconstructs more vertex-level accurate (MPVE) meshes than the off-the-shelf neural model, DECA. 
%   % 
%   % $\emph{Abbr.}$ lmk: landmark, vtx: vertex.
%   }
%   % \vspace{-3mm}
%   % }
%   \label{tab:vocaset}
% \end{table}


%%%%%%Current Version
\begin{table}[t!]
  \centering
  \resizebox{1\linewidth}{!}{
  \begin{tabular}{l cccc}
  \toprule
  % &\multicolumn{2}{c}{Methods} \\
  % \cmidrule(lr){2-3} 
  Method & CVD $\downarrow$ &  MSI\textsubscript{3D, lmk} $\uparrow$\ & MSI\textsubscript{3D, vtx} $\uparrow$ & MPVE [\emph{mm}] $\downarrow$ \\
  \cmidrule(lr){1-5} 
  DECA~\cite{DECA:Siggraph2021} & 0.440 & 0.005 & 0.006 & 39.9\\
  NeuFace (ours) & \textbf{0.322}  & \textbf{0.379} &\textbf{ 0.530}& \textbf{31.2}\\
  \bottomrule
  \end{tabular}}
  \caption{\textbf{Accuracy of NeuFace optimization on motion capture dataset w/ GT.}
  % \kim{
  Given the ground-truth meshes of multi-view motion captured dataset, VOCASET, our NeuFace optimization reconstructs \kim{spatio-temporally consistent and} more vertex-level accurate (MPVE) meshes than the off-the-shelf neural model, DECA. 
  % 
  % $\emph{Abbr.}$ lmk: landmark, vtx: vertex.
  }
  % \vspace{-3mm}
  % }
  \label{tab:vocaset}
\end{table}

